Separation and Estimation of Periodic/Aperiodic State

Periodicity and aperiodicity can exist in a state simultaneously and typically become quasi-periodicity and quasi-aperiodicity in a dynamically changing state. The quasi-periodic and quasi-aperiodic states existing in the periodic/aperiodic state mostly correspond to different phenomena and require different controls. For separation control of these states, this paper defines the periodic/aperiodic, quasi-periodic, and quasi-aperiodic states to construct a periodic/aperiodic separation filter that separates the periodic/aperiodic state into the quasi-periodic and quasi-aperiodic states. Based on these definitions, the linearity of periodic-pass and aperiodic-pass functions and the orthogonality of quasi-periodic and quasi-aperiodic state functions are proved. Subsequently, the periodic/aperiodic separation filter composed of periodic-pass and aperiodic-pass filters that realize the periodic-pass and aperiodic-pass functions is designed and integrated with a Kalman filter for estimation of the quasi-periodic and quasi-aperiodic states.

==> text/biography.tex <==
\begin{IEEEbiography}{Hisayoshi Muramatsu}
received the B.E. degree in system design engineering from Keio University, Yokohama, Japan, in 2016.
Since 2016, he has been in the Master's course at Keio University, Yokohama, Japan.
His research interests include motion control and mechatronics.
He is a Student Member of IEEJ, as well as a Student Member of the IEEE.
\end{IEEEbiography}
\begin{IEEEbiography}{Seiichiro Katsura}
received the B.E. degree in system design engineering and the M.E. and Ph.D.
degrees in integrated design engineering from Keio University, Yokohama, Japan, in 2001, 2002 and 2004, respectively.
%
From 2003 to 2005, he was a Research Fellow of the Japan Society for the Promotion of Science (JSPS).
From 2005 to 2008, he was with Nagaoka University of Technology, Nagaoka, Japan.
Since 2008, he has been with Keio University.
His research interests include abstraction, human support, wave system, and systems energy conversion.
%
Prof. Katsura serves as an Associate Editor of the IEEE Transactions on Industrial Electronics.  He
was the recipient of the IEEE Industrial Electronics  Society Best Conference Paper Award in 2012
and JSPS Prize in 2016.
\end{IEEEbiography}

